A Data-Efficient Deep Learning Framework for Segmentation and Classification of Histopathology Images

The current study of cell architecture of inflammation in histopathology images commonly performed for diagnosis and research purposes excludes a lot of information available on the biopsy slide. In autoimmune diseases, major outstanding research questions remain regarding which cell types participate in inflammation at the tissue level, and how they interact with each other. While these questions can be partially answered using traditional methods, artificial intelligence approaches for segmentation and classification provide a much more efficient method to understand the architecture of inflammation in autoimmune disease, holding great promise for novel insights. In this paper, we empirically develop deep learning approaches that use dermatomyositis biopsies of human tissue to detect and identify inflammatory cells. Our approach improves classification performance by 26% and segmentation performance by 5%. We also propose a novel post-processing autoencoder architecture that improves segmentation performance by an additional 3%.

==> claassification_recall.tex <==
\subsection{Recall for Classification}

Since the dataset, was unballanced looking at the recall values would also be helpful as recall is semantically equivalent to the balanced multi-class accuracy.

\begin{table}[]
\begin{center}
\caption{We report the F1 score for with Imagenet initialization for latest set of CNNs and Transformers. We observe the usual trend of increasing Imagenet performance with increasing size of the model is not followed. Overall the best performance is achieved by nfnet-f3 for CNNs. Overall, out of all the tested architectures Swin Transformer Base with Patch 4 and Window 12 performs the best.}
\label{table:allcnn}
\begin{tabular}{ll}
\hline\noalign{\smallskip}
\textbf{Model}    & \textbf{Test F1-Score} \\
\hline\noalign{\smallskip}
Resnet-18         & 0.8635±0.0087          \\
Resnet-34         & 0.82765±0.0073         \\
Resnet-50         & 0.8499±0.007           \\
Resnet-101        & 0.871±0.009            \\
Efficient-net B0  & 0.8372±0.0007          \\
Efficient-net B1  & 0.8346±0.0026          \\
Efficient-net B2  & 0.828±0.00074          \\
Efficient-net B3  & 0.8369±0.0094          \\
Efficient-net B4  & 0.8418±0.0009          \\
Efficient-net B5  & 0.8463±0.00036         \\
Efficient-net B6  & 0.8263±0.00147         \\
Efficient-net B7  & 0.8129±0.001           \\
nfnet-f0          & 0.82035±0.007          \\
nfnet-f1          & 0.834±0.007            \\
nfnet-f2          & 0.8652±0.0089          \\
nfnet-f3          & 0.8898±0.0011          \\
nfnet-f4          & 0.8848±0.0109 \\
nfnet-f5 & 0.8161±0.0074          \\
nfnet-f6 & 0.8378±0.007           \\
ConvNext-tiny     & 0.81355±0.0032         \\
ConvNext-small    & 0.84795±0.00246        \\
ConvNext-base     & 0.80675±0.002          \\
ConvNext-large    & 0.8452±0.000545       \\
Swin Transformer large\\ (Patch 4 Window 12)\ & 0.8839±0.001           \\
Swin Transformer Base\\ (Patch 4 Window 12)\  & \textbf{0.891±0.0007}           \\
Vit-Base/16                                                                          & 0.8426±0.007           \\
Vit-Base/32                                                                          & 0.8507±0.0079          \\
Vit-large/16                                                                         & 0.80495±0.0077         \\
Vit-large/32                                                                         & 0.845±0.0077          \\
\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}


==> extra.tex <==
%%%%%Older Intro
\section{Introduction}
The world plunged into a great unknown with the Covid-19 pandemic. The race to discover the cure or some remedy to this global health crisis proves better understanding of human disease and virology are required. Ever since the spread of the coronavirus, immunity related diseases have been in the spotlight. But despite this certain class of diseases such as autoimmune diseases have been traditionally extremely under represented within the application of artificial intelligence domain. Median dataset size available in the field range between 99-540 \cite{stafford2020systematic} as opposed to other datasets which are easily available in the range of few thousands to a few hundered thousand \cite{yang2021medmnist}.

With this paper out aim is to draw more attention to autoimmune diseases and more specifically helping practitioners with the help of developments made in artificial intelligence and deep learning. With this paper we (i)improve upon existing method for classification and segmentation of autoimmune diseases images with 25\% improvement for classification and 5\% overall for segmentation. (ii) study the effect of using different initialisation. (iii) adding auto-encoder for post processing and using image reconstruction loss improves segmentation performance by 3\%.

%%%from rd.tex%%%%
\subsubsection{Effect of different weights} To understand the Effect of different initialization, instead of using highly specialized weights like Brain-MRI segmentation used by previous students. We use the widely available Imagenet weights for initialization, which have been credited to better weight scaling and faster convergence, based on the findings from \cite{raghu2019transfusion}. We also two extensions of imagent training with (i) Noisy student trained encoders \cite{xie2020self}. Noisy Student Training extends the idea of self-training and distillation with the use of equal-or-larger student models, and noise such as dropout, stochastic depth,
and data augmentation via RandAugment is added to the student during learning so
that the student generalizes better than the teacher. First, an EfficientNet model is trained on labelled images and is used as a teacher to generate pseudo labels for 300M unlabeled images. We then train a larger EfficientNet as a student model on the combination of labelled and
pseudo-labelled images. This helps reduce the error rate, increases robustness and improves performance over the existing state-of-the-art on Imagenet. 

(ii)AdvProp training, which banks on Adversarial examples, which are commonly viewed as a threat
to ConvNets. In \cite{xie2020adversarial} they present an opposite perspective: adversarial examples can be used to improve image recognition models. They treat adversarial examples as additional examples, to prevent overfitting. It performs better
when the models are bigger. This improves upon performance for various imagenet and imagenet subset benchmarks. 

Since, originally all these were developed for the efficient net family of encoder, we used them for bench marking. We present their results in Table~\ref{table:segweights}

\begin{table}[!h]
\begin{center}
\caption{Using different initialisation, we see the performance of different encoders of efficient net family on Unet. We report the IoU over test set in the following table.
We observe that while performance gains for smaller models, Imagenet initialisation works better for larger models. Also, the fact that Advprop and noisy are not readily available for all models, hence the choice of Imagenet still dominates. }
\label{table:segweights}

\begin{tabular}{llll}
\hline\noalign{\smallskip}
\textbf{Encoder} & \textbf{Imagenet} & \textbf{Advprop} & \textbf{Nosiy}  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
B0               & 0.3785            & 0.3895           & \textbf{0.4081} \\
B1               & 0.3301            & 0.2330           & \textbf{0.3817} \\
B2               & 0.2235            & 0.3823           & \textbf{0.4154} \\
B3               & \textbf{0.3982}   & 0.3722           & 0.3509          \\
B4               & 0.3831            & \textbf{0.4366}  & 0.4333          \\
B5               & \textbf{0.4056}   & 0.3910           & 0.3806          \\
B6               & \textbf{0.4001}   &  0.3807                 & 0.3941          \\
B7               &  \textbf{0.3631}                 & 0.3543                 & 0.3308                \\
\hline
\end{tabular}
\end{center}
\end{table}

We also present results for classification with different initialisation in % TODO:add table.

Since, Imagenet initialisation provide the best performance, so keeping inline we also benchmark on the gold-standard of CNNs in computer vision - the resnet family\cite{he2015deep}. We present their result in 
Table~\ref{table:resnet}.

\begin{table}[!h]
\begin{center}
\caption{Using different initialisation, we see the performance of different encoders of efficient net family on Unet.
We observe that while performance gains for smaller models, Imagenet initialisation works better for larger models. Also, the fact that Advprop and noisy are not readily available for all models, hence the choice of Imagenet still dominates. }
\label{table:resnet}

\begin{tabular}{llll}
\hline\noalign{\smallskip}
\textbf{Encoder} & \textbf{Test IoU} & \textbf{Params(M)} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
resnet18         & 0.4347            & 11.69           \\
resnet34         & 0.4774            & 21.80           \\
resnet50         & 0.3798            & 25.56           \\
resnet101        & 0.3718            & 44.55           \\
\hline
\end{tabular}
\end{center}
\end{table}



 \subsubsection{Effect of Initialisation} As already mentioned in section 5.1, in addition to the traditional Imagenet initialisation we use extensions of Imagenet training with Advprop and Noisy student training.
 Since, these experiemnts were conducted for the efficient net family of encoder we report their performance in Table \ref{table:effnet}
 
 \begin{table}[]
 \begin{center}
\caption{We report the F1 score for different initialisations for the Efficient net family of encoders. We report the average of 5 fold runs on the test set. We observe that 0.8463 is the peak with Imagenet, 0.843 with Advprop and 0.8587 with Noisy student initialisation.}
\label{table:effnet}
\begin{tabular}{llll}
\hline\noalign{\smallskip}
\textbf{Encoder} & \textbf{Imagenet}       & \textbf{Advprop}       & \textbf{Noisy Student} \\
\hline\noalign{\smallskip}
B0               & 0.8372± 0.0007          & \textbf{0.8416±0.0008} & 0.839±0.0008           \\
B1               & 0.8346±0.0026           & 0.8367±0.0007          & \textbf{0.8478±0.0014} \\
B2               & 0.828±0.00074           & \textbf{0.843±0.00138} & 0.8430±0.0012          \\
B3               & 0.8369±0.0094           & 0.85138±0.00135        & \textbf{0.8587±0.007}  \\
B4               & \textbf{0.8418±0.0009}  & 0.82135±0.00058        & 0.8377±0.00032         \\
B5               & \textbf{0.8463±0.00036} & 0.8133±0.002           & 0.8326±0.00066         \\
B6               & \textbf{0.8263±0.00147} & 0.8237±0.004           & 0.8233±0.0065          \\
B7               & 0.8129±0.001            & 0.8132±0.004           & \textbf{0.8257±0.0008} \\
\hline\noalign{\smallskip}
\end{tabular}
\end{center}
\end{table}

From table \ref{table:effnet} we observe that for most cases Nosiy student and Imagenet initialisations yield the best results.Although this gain is only around 1\%. This is overshadowed by the excessive computational power required to get the noisy student weights as opposed to Imagenet weights. Hence we stick to Imagenet weights due to their ease of availability and relatively small gains with other weights. 


%%%%Table from Rd.tex

\begin{table}[!ht]
\begin{center}
\caption{This table shows the IoU score on test set for Unet and Unet++ architectures. We compare results using auto-encoder with ReLU and GELU activations. For the same we observe that GELU auto-encoders improve the performance in all most all cases with a consistent gain of 3\% in IoU. We also observe that the nature of gain is also consistent with Autoencoder with ReLU activation working better with Resnet-50 for both Unet and Unet++. }
\label{table:unetae}
\begin{tabular}{lllll}
\hline\noalign{\smallskip}
\textbf{Encoder} & \multicolumn{2}{c}{\textbf{Unet}}                                                                                          & \multicolumn{2}{c}{\textbf{Unet++}}                                                                                         \\
\hline
\textbf{}        & \textbf{\begin{tabular}[c]{@{}l@{}}Without\\ AE\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}With\\ AE\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Without\\ AE\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}With \\ AE\end{tabular}} \\
\hline\noalign{\smallskip}
Resnet 18        & 0.4347                                                        & \textbf{0.4608}                                            & \textbf{0.5274}                                               & 0.4177                                                      \\
Resnet 34        & \textbf{0.4774}                                               & 0.4467                                                     & 0.3745                                                        & \textbf{0.4535}                                             \\
Resnet 50        & 0.3798                                                        & \textbf{0.4187}                                            & 0.4236                                                        & \textbf{0.4685}                                             \\
Resnet 101       & 0.3718                                                        & \textbf{0.4074}                                            & \textbf{0.4311}                                               & 0.4265   \\
\hline\noalign{\smallskip}
\end{tabular}
\end{center}  
\end{table}

